Constructing Unrestricted Adversarial Examples with Generative Models

Adversarial examples are typically constructed by perturbing an existing data point within a small matrix norm, and current defense methods are focused on guarding against this type of attack. In this paper, we propose unrestricted adversarial examples, a new threat model where the attackers are not restricted to small norm-bounded perturbations. Different from perturbation-based attacks, we propose to synthesize unrestricted adversarial examples entirely from scratch using conditional generative models. Specifically, we first train an Auxiliary Classifier Generative Adversarial Network (AC-GAN) to model the class-conditional distribution over data samples. Then, conditioned on a desired class, we search over the AC-GAN latent space to find images that are likely under the generative model and are misclassified by a target classifier. We demonstrate through human evaluation that unrestricted adversarial examples generated this way are legitimate and belong to the desired class. Our empirical results on the MNIST, SVHN, and CelebA datasets show that unrestricted adversarial examples can bypass strong adversarial training and certified defense methods designed for traditional adversarial attacks.

==> app.tex <==
\newpage
\appendix

\section{Analysis of imperfect generators}\label{app:proof}
In this section, we give one possible explanation for why in practice generative models can create adversarial examples that fool classifiers. We will now assume that generators not always generate legitimate images from the desired class. We will argue that, under some strong assumptions, when the classifier's prediction contradicts the generator's label conditioning, it is more likely for the classifier to make a mistake, rather than the generator generates an incorrect image.

In order to make our argument, we first need \propref{prop:main}:
\begin{proposition}\label{prop:main}
	Let $\mbf{W}\in\mbb{R}^{n \times m}$ be a random variable. Assume each entry of $\mbf{W}$ is bounded, \ie, $|w_{ij}| \leq K$ for all $i$ and $j$. Furthermore, we assume $w_{ij}$ are mutually independent, and $|\mbb{E}[w_{ij}]| \leq \tau$. Then, with probability $1 - \delta$, the following bound holds
	\begin{align}
	\frac{1}{n}\max_{\norm{\Delta \mbf{x}}_\infty \leq \epsilon}\norm{\mbf{W} \cdot \Delta \mbf{x}}_1 \leq 4 \epsilon K \sqrt{\frac{m\big(m \log 2 + \log \frac{1}{\delta}\big)}{n}} + \epsilon \tau m. \label{eqn:main}
	\end{align}
\end{proposition}

\begin{proof}
	Let $\Wb = (\wb_1^\intercal, \wb_2^\intercal, \cdots, \wb_n^\intercal)^\intercal$, where $\wb_i$ represents the $i$-th row vector of $\Wb$. In order to bound $\max_{\norm{\Delta \xb}_\infty \leq \epsilon} \norm{\Wb \Delta \xb}_1$, we first bound $\norm{\Wb \Delta \xb}_1$ for any fixed vector $\Delta\xb$ from the ball $\mcal{B}_\epsilon :=\{ \xb \mid \norm{\xb}_\infty \leq \epsilon \}$ and then apply union bound. Note that $\norm{\Wb \Delta \xb}_1$ can be written as the sum of $n$ terms, \ie,  $\norm{\Wb \Delta \xb}_1 = \sum_{i=1}^n |\wb_i^\intercal \Delta \xb|$, where each term $\wb_i^\intercal \Delta \xb$ can be bounded using McDiarmid's inequality~\cite{tao2012topics}
	\begin{align}
	\mbb{P}\left( \sum_{j=1}^m w_{ij} (\Delta x)_j - M_i \geq \lambda\right) \leq \exp\left( \frac{-\lambda^2}{2 m K^2 \epsilon^2} \right)\label{eqn:sg},
	\end{align}
	where $M_i = \sum_{j=1}^m \mbb{E}[w_{ij} (\Delta x)_j] \leq \epsilon \tau m$, according to the theorem's assumption. 
	
	From \eqref{eqn:sg} we conclude the random variable $\wb_i^\intercal\Delta\xb - M_i$ is sub-Gaussian~\cite{rigollet2015high}, hence
	\begin{align*}
	&\mbb{E}\left[ \exp(s|\wb_i^\intercal \Delta \xb - M_i|) \right] \leq \exp \left( 4 s^2 mK^2 \epsilon^2 \right)\\
	\Rightarrow & \mbb{E} \left[  \exp\left( s\sum_{i=1}^n |\wb_i^\intercal \Delta \xb - M_i| \right) \right] \leq \exp(4s^2 nmK^2 \epsilon^2).
	\end{align*}
	With Markov inequality~\cite{tao2012topics}, we obtain
	\begin{align}
	\mbb{P}\left(\sum_{i=1}^n |\wb_i^\intercal \Delta \xb - M_i| \geq \lambda\right)  \leq \exp(4s^2 nmK^2 \epsilon^2 - s \lambda ).\label{eqn:markov1}
	\end{align}
	Because \eqref{eqn:markov1} holds for every $s\in\mbb{R}$, we can optimize $s$ to get the tightest bound
	\begin{align*}
	&\mbb{P}\left(\sum_{i=1}^n |\wb_i^\intercal \Delta \xb - M_i| \geq \lambda\right)\leq \exp\left( -\frac{\lambda^2}{16 nmK^2 \epsilon^2} \right)\\
	\Rightarrow&
	\mbb{P} \left(\norm{\Wb \Delta \xb}_1 \geq \lambda+ \sum_{i=1}^n |M_i|\right)\leq \exp\left( -\frac{\lambda^2}{16 nmK^2 \epsilon^2} \right)\\
	\Rightarrow&
	\mbb{P} \left(\norm{\Wb \Delta \xb}_1 \geq \lambda + \tau \epsilon n m\right)\leq \exp\left( -\frac{\lambda^2}{16 nmK^2 \epsilon^2} \right).\label{eqn:part1}
	\end{align*}
	Now we are ready to apply union bound to control $\max_{\Delta \xb \in \mcal{B}_\epsilon} \norm{\Wb \Delta \xb}_1$. Although $\mcal{B}_\epsilon$ is an infinite set, we only need to consider a finite set of vertices $\mcal{V}_\epsilon:= \{ \xb \mid x_i \in \{-\epsilon, \epsilon\},~\forall i = 1,2,\cdots,m \}$. To see this, assume $\xb^* = \argmax_{\xb\in\mcal{S}_\epsilon} \norm{\Wb \xb}_1$ but $\xb^* \not\in \mcal{V}_\epsilon$. Because $\mcal{B}_\epsilon$ is a convex polytope with vertices $\mcal{V}_\epsilon$, we have $\xb^* = \sum_{i=1}^{2^m} \lambda_i \vb_i$, where $\lambda_i\in[0,1]$, $\sum_{i=1}^{2^m} \lambda_i = 1$ and $\vb_i$ denotes the $i$-th vertex in $\mcal{V}_\epsilon$. By triangle inequality we have
	\begin{align*}
	\norm{\Wb \xb^*}_1 &= \norm{\sum_{i=1}^{2^m}\lambda_i \Wb \vb_i}_1\\
	&\leq \sum_{i=1}^{2^m} \lambda_i \norm{\Wb \vb_i}_1\\
	&\leq \left(\sum_{i=1}^{2^m}\lambda_i\right) \max_{i\in[0,2^m]} \norm{\Wb \vb_i}_1\\
	&= \max_{i\in[0,2^m]} \norm{\Wb \vb_i}_1 \leq \norm{\Wb \xb^*}_1.
	\end{align*}
	Let $\vb^* := \argmax_{\vb_i, i \in [0,2^m]} \norm{\Wb\vb_i}_1$. From the above derivation we conclude $\norm{\Wb \vb^*}_1 = \norm{\Wb \xb^*}_1$ and therefore it is sufficient to only consider $\mcal{V}_\epsilon$ for union bound:
	\begin{align*}
	\mbb{P} \left(\max_{\Delta\xb \in \mcal{S}_\epsilon}\norm{\Wb \Delta \xb}_1 \geq \lambda +  \epsilon \tau n m\right)
	&= \mbb{P} \left(\max_{\Delta\xb \in \mcal{V}_\epsilon}\norm{\Wb \Delta \xb}_1 \geq \lambda + \epsilon \tau n m\right)\\
	&\leq |\mcal{V}_\epsilon| \mbb{P}\left(\norm{\Wb \Delta \xb}_1 \geq \lambda + \epsilon \tau n m\right) \tag{\text{Union Bound}}\\
	&\leq 2^m \exp\left( -\frac{\lambda^2}{16 nmK^2 \epsilon^2} \right).
	\end{align*}
	In other words, with probability $1-\delta$,
	\begin{align*}
	\max_{\Delta\xb \in \mcal{S}_\epsilon}\norm{\Wb \Delta \xb}_1 \leq 4 K\epsilon \sqrt{mn\left(m\log 2 +\log \frac{1}{\delta}\right)} + \epsilon \tau nm,
	\end{align*}
	and the statement of our theorem gets proved.
\end{proof}
\subsubsection*{Remarks}
Intuitively, \propref{prop:main} characterizes the robustness of a ``typical'' linear function as a function of its input and output dimensions. Specifically, it becomes more robust as the output dimensionality increases. This is based on the observation that when the input dimension $m$ is fixed, the average maximum perturbation of its output ($\frac{1}{n}\max_{\norm{\Delta\mbf{x}}_{\infty}\leq \epsilon}\norm{\mbf{W}\cdot \Delta \mbf{x}}$) is upper bounded by $O(n^{-\frac{1}{2}})$, which decreases as $n$ gets larger.


Now we show how to apply \propref{prop:main} to a binary classification problem.
\paragraph{Notations}
Let $s(x)$ be the score function of interest, where $x \in \mbb{R}^n$ is an input image. Let the targeted classifier be $f(x) = \operatorname{sign}(s(x))$. Given a latent code $z \in \mbb{R}^m$ and a conditioning label $y \in \{-1, 1\}$, our generative model $g$ produces an image $g(z, y) \in \mbb{R}^n$. We denote the prior distribution of $z$ as $P_z$. Additionally, let $\mbf{J}_{g(z_0, y_0)} \in \mbb{R}^{n \times m}$ be the Jacobian of $g(z, y)$ \wrt $z$, when $z = z_0$ and $y = y_0$. We similarly define $\mbf{J}_{s(g(z_0, y_0))} \in \mbb{R}^{1 \times m}$ to be the Jacobian of $s(g(z, y))$. When we fix $y_0$ and treat $z_0$ as a random variable with distribution $P_z$, $\mbf{J}_{g(z_0, y_0)}$ and $\mbf{J}_{s(g(z_0, y_0))}$ become random matrices, which we denote as $\mbf{J}_g \in \mbb{R}^{n \times m}$ and $\mbf{J}_s \in \mbb{R}^{1\times m}$. Finally, let $J_{ij}^g$ and $J_{ij}^s$ be the $i, j$-th entry of $\mbf{J}_g$ and $\mbf{J}_s$ respectively.

\paragraph{Assumptions}
We make the following assumptions.
\begin{enumerate}
	\item $\{J_{ij}^g \mid 1\leq  i\leq n, 1\leq j \leq m\}$ and $\{ J_{ij}^s \mid i = 1, 1\leq j\leq m\}$ are both mutually independent.
	\item $\max_{1 \leq i \leq n, 1\leq j \leq m} |J_{ij}^g| \leq K$ and $\max_{i =1, 1\leq j\leq m} |J_{ij}^s| \leq K$.
	\item $\max_{1 \leq i \leq n, 1\leq j\leq m} |\mbb{E}[J_{ij} ^ g]| \leq \tau$ and $\max_{i=1, 1\leq j\leq m} |\mbb{E}[J_{ij}^s]| \leq \tau$.
	\item $\tau \ll K$.
	\item The gap between L.H.S. and R.H.S. of \eqref{eqn:main} in \propref{prop:main} is the same.
	\item $x$ and $x'$ have the same label if $\norm{x - x'}_1$ is small.
\end{enumerate}
\paragraph{Conclusion}
With high probability, when sampling $z^0 \sim P_z$ randomly, we have
\begin{align}
\max_{\|\delta_z\|_\infty \leq \epsilon}\frac{1}{n} \|g(z^0 + \delta_z, y) - g(z^0, y)\|_1 \ll \max_{\|\delta_z\|_\infty \leq \epsilon}|s(g(z^0 + \delta_z, y)) - s(g(z^0, y))|.\label{eqn:goal}
\end{align}
Consider our algorithm of creating generative adversarial examples, where we search $z$ within $\| z - z^0\|_\infty \leq \epsilon$ so that $f(g(z, y)) \neq o(g(z, y))$. From \eqref{eqn:goal} we know that the worst perturbation per dimension of $g(z, y)$ is usually much smaller than that of $s(g(z, y))$. If $o(g(z^0, y)) = y$, this means $o(g(z, y)) = y$ is more likely to hold than $o(g(z, y)) = f(g(z, y))$ (according to Assumption 6), which means $f$ is more likely to make the mistake.

\paragraph{Arguments for conclusion}
Both sides of \eqref{eqn:goal} are hard to quantify in general (actually computing the L.H.S. is NP-hard~\cite{rohn2000computing}). We choose to rely on Assumption 5 and propose to compare their upper bounds.

Let $z^0 \sim P_z$ and $\|\delta_z \|_\infty \leq \epsilon$. We can approximate $\| g(z^0 + \delta_z, y) - g(z^0, y)\|_1 \approx \|\mbf{J}_{g(z^0, y)} \delta_z\|_1$ and $|s(g(z^0 + \delta_z, y)) - s(g(z^0, y))| \approx |\mbf{J}_{s(g(z^0, y))}\delta_z|$. If all assumptions are true, we can apply \propref{prop:main} and see that the first term on R.H.S. of \eqref{eqn:main} dominates the upper bound. Since $\mbf{J}_g \in \mbb{R}^{n\times m}$ and $\mbf{J}_s \in \mbb{R}^{1\times m}$, it is clear that the upper bound for $\max_{\|\delta_z\|_\infty \leq \epsilon}\frac{1}{n} \|g(z^0 + \delta_z, y) - g(z^0, y)\|_1$ is much smaller than that of $\max_{\|\delta_z\|_\infty \leq \epsilon}|s(g(z^0 + \delta_z, y)) - s(g(z^0, y))|$, especially when $n \gg 1$. This justifies our conclusion.



\section{Pseudocode}\label{app:code}

\begin{algorithm}[ht]
	\caption{Generative Adversarial Example Targeted Attack}
	\label{alg:attack}
	\begin{algorithmic}[1] % The number tells where the line numbering should start
		\Procedure{Attack}{$y_\text{target}, y_\text{source}, f, \theta, \phi, \epsilon, \epsilon_\text{attack}, \lambda_1, \lambda_2,\alpha, T$}
		\State Define $\mathcal{L}(z, \tau\mathbin{;} z^0, y_\text{target}, y_\text{source}, f, \theta, \phi, \epsilon, \epsilon_\text{attack}, \lambda_1, \lambda_2)$
		\begin{align*}
		\mathcal{L} = 
		&-\log f(y_\text{target} \mid g_\theta(z, y_\text{source}) + \epsilon_\text{attack}\tanh(\tau)) +\lambda_1 \cdot \frac{1}{m}\sum_{i=1}^m \max\{|z_i - z_i|, \epsilon\}\\
		&\hspace{0.5cm}
		-\lambda_2 \cdot \log c_\phi(y_\text{source} \mid g_\theta(z, y_\text{source}) + \epsilon_\text{attack}\tanh(\tau))
		\end{align*}
		\State Initialize $x_\text{attack} \gets \varnothing$
		\While{$x_\text{attack} = \varnothing$}
		\State Sample $\tau \sim \mathcal{N}(0, 1)$
		\State Sample $z^0 \sim \mathcal{N}(0, 1)$
		\State Initialize $z \gets z^0$
		\For{$i = 1\ldots T$}
		\State Update $z \gets z - \alpha \cdot \frac{\partial\mathcal{L}(z, \tau)}{\partial z}$ \Comment{$\alpha$ is the learning rate.}
		\State $\Delta \gets \frac{\partial\mathcal{L}(z, \tau)}{\partial \tau}$                                 \State Update $\tau \gets \tau - \alpha \cdot \frac{\Delta}{\|\Delta\|}$ \Comment{We found gradient normalization to be effective}
		\EndFor
		\State $x \gets g_\theta(z, y_\text{source}) + \epsilon_\text{attack}\tanh(\tau)$
		\If{$y_\text{target} = \argmax_y p(f(x) = y)$}
		\State $x \gets x_\text{attack}$
		\EndIf
		\EndWhile
		\State \textbf{return} $x_\text{attack}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\section{Detailed experimental settings}\label{app:arch}
\paragraph{Datasets} The datasets used in our experiments are MNIST~\cite{lecun1989backpropagation}, SVHN~\cite{netzer2011reading}, and CelebA~\cite{liu2015faceattributes}. Both MNIST and SVHN are images of digits. MNIST contains 60000 28-by-28 gray-scale digits in the training set, and 10000 digits in the test set. In SVHN, there are 73257 32-by-32 images of house numbers (captured from Google Street View) for training, 26032 images for testing, and 531131 additional images as extra training data. For CelebA, there are 202599 celebrity faces, each of which has 40 binary attribute annotations. We group the face images according to female/male, and focus on gender classification. The first 150000 images are split for training and the rest are used for testing.

\paragraph{Adversarial training} Regarding adversarial training, we directly use the weights provided by~\cite{madry2017towards} for MNIST. For other tasks, we combine the techniques from~\cite{madry2017towards} and~\cite{kurakin2016adversarialscale}. More specifically, suppose pixel space is $[0, 255]$. We first sample $\epsilon$ from $\mcal{N}(0, 8)$, take the absolute value and truncate it to $[0, 16]$, after which we use PGD with $\epsilon$ and iteration number $\lfloor \min(\epsilon + 4, 1.25\epsilon) \rfloor$ to generate adversarial examples for adversarial training. As suggested in~\cite{kurakin2016adversarialscale}, this has the benefit of making models robust to attacks with different $\epsilon$.

\paragraph{Model architectures} 
For the AC-GAN architecture, we mostly follow the best designs tested in~\cite{gulrajani2017improved}. Specifically, we adapted their AC-GAN architecture on CIFAR-10 for our experiments of MNIST and SVHN, and used their AC-GAN architecture on 64$\times$64 LSUN for our CelebA experiments. Since MNIST digits have lower resolution than CIFAR-10 images, we reduced one residual block in the generator so that the output shape is smaller, and reduced the channels of output from 3 to 1. The other components of AC-GAN, including architecture of the discriminator and auxiliary classifier, are all the same as described in~\cite{gulrajani2017improved}.

For classifier architectures, we obtained networks and weights from authors of~\cite{madry2017towards, raghunathan2018certified,kolter2017provable} so that we can be consistent with their papers. The ResNet architectures used for SVHN, CelebA and transferability experiments are shown in \tabref{tab:arch}.
\begin{table}
	\caption{Hyperparameters of generative adversarial attacks. Notations are the same as in \agref{alg:attack}. $^*$Target class is ``Male''. $^\dagger$Target class is ``Female''.}\label{tab:hyperparams}
	\centering
	\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{cccccccccc}
			\Xhline{3\arrayrulewidth} \bigstrut
			Datasets & Classifier & Targeted & Noise & $\lambda_1$ & $\lambda_2$ & $\epsilon$ & $\epsilon_\text{attack}$ & $\alpha$ & $T$ \\
			\Xhline{1\arrayrulewidth}\bigstrut
			MNIST & Madry Net~\cite{madry2017towards} & Yes & No & 50 & 0 & 0.1 & 0 & 1 & 500\\
			MNIST & Madry Net~\cite{madry2017towards} & Yes & Yes & 50 & 0 & 0.1 & 0.3 & 1 & 500\\
			MNIST & \cite{raghunathan2018certified} & No & No & 100 & 0 & 0.1 & 0 & 10 & 100\\
			MNIST & \cite{kolter2017provable} & No & No & 100 & 0 & 0.1 & 0 & 1 & 100\\
			SVHN & ResNet & Yes & No & 100 & 100 & 0.01 & 0 & 0.1 & 200 \\
			SVHN & ResNet & Yes & Yes & 100 & 100 & 0.01 & 0.03 & 0.5 & 300 \\
			CelebA$^*$ & ResNet & Yes & No & 100 & 100 & 0.001 & 0 & 1 & 200\\
			CelebA$^*$ & ResNet & Yes & Yes & 100 & 100 & 0.001 & 0.03 & 1 & 200\\
			CelebA$^\dagger$ & ResNet & Yes & No & 100 & 100 & 0.1 & 0 & 0.1 & 200 \\
			CelebA$^\dagger$ & ResNet & Yes & Yes & 100 & 100 & 0.1 & 0.03 & 0.1 & 200\\
			\Xhline{3\arrayrulewidth}
		\end{tabular}
	\end{adjustbox}
\end{table}

\begin{table}
	\small
	\centering
	\caption{ResNet Classifier Architecture. We set the base number of feature maps to $m = 4$ for MNIST and $m = 16$ for SVHN and CelebA.}\label{tab:arch}
	\begin{tabular}{l|c|c}
		\Xhline{3\arrayrulewidth}\bigstrut
		\bf Name & \bf Configuration & \bf Replicate Block \\
		\hline\bigstrut
		Initial Layer & 
		$3 \times 3$ conv. $m$ maps. $1 \times 1$ stride. & --- \\
		\hline\bigstrut
		\multirow{5}{*}{Residual Block 1} & batch normalization, leaky relu & \multirow{5}{*}{$\times 10$} \\
		& $3 \times 3$ conv. $m$ maps. $1 \times 1$ stride & \\
		& batch normalization, leaky relu & \\
		& $3 \times 3$ conv. $m$ maps. $1 \times 1$ stride & \\
		& residual addition & \\
		\hline\bigstrut
		\multirow{5}{*}{Resize Block 1} & batch normalization, leaky relu & \multirow{5}{*}{---}\\
		& $3 \times 3$ conv. $2m$ maps. $2 \times 2$ stride & \\
		& batch normalization, leaky relu & \\
		& $3 \times 3$ conv. $2m$ maps. $1 \times 1$ stride & \\
		& average pooling, padding & \\
		\hline\bigstrut
		\multirow{5}{*}{Residual Block 2} & batch normalization, leaky relu & \multirow{5}{*}{$\times 9$} \\
		& $3 \times 3$ conv. $2m$ maps. $1 \times 1$ stride & \\
		& batch normalization, leaky relu & \\
		& $3 \times 3$ conv. $2m$ maps. $1 \times 1$ stride & \\
		& residual addition & \\
		\hline\bigstrut
		\multirow{5}{*}{Resize Block 2} & batch normalization, leaky relu & \multirow{5}{*}{---}\\
		& $3 \times 3$ conv. $4m$ maps. $2 \times 2$ stride & \\
		& batch normalization, leaky relu & \\
		& $3 \times 3$ conv. $4m$ maps. $1 \times 1$ stride & \\
		& average pooling, padding & \\
		\hline\bigstrut
		\multirow{5}{*}{Residual Block 3} & batch normalization, leaky relu & \multirow{5}{*}{$\times 9$} \\
		& $3 \times 3$ conv. $4m$ maps. $1 \times 1$ stride & \\
		& batch normalization, leaky relu & \\
		& $3 \times 3$ conv. $4m$ maps. $1 \times 1$ stride & \\
		& residual addition & \\
		\hline\bigstrut
		Pooling Layer & batch normalization, leaky relu, average pooling & ---\\
		\hline
		\bigstrut
		Output Layer & $10$ dense, softmax & ---\\
		\Xhline{3\arrayrulewidth}
		%\bigstrut
	\end{tabular}
\end{table}

\paragraph{Hyperparameters of attacks}
\tabref{tab:hyperparams} shows our hyperparameters of all generative adversarial attacks used in this paper, following the same notations in arguments of \agref{alg:attack}.




\clearpage
\section{Additional samples}\label{app:samples}
\vspace*{\fill}
\begin{figure}[H]
	\centering
	\subfigure[Extended plot for untargeted attacks against~\cite{raghunathan2018certified}.]{
	\includegraphics[width=\textwidth]{mnist_aditi_adv_untargeted_plot_larger.png}}

	\subfigure[Extended plot for untargeted attacks against~\cite{kolter2017provable}.]{
		\includegraphics[width=\textwidth]{mnist_zico_adv_untargeted_plot_larger.png}
	}
	\caption{(Extended plot of \figref{fig:3}) Random samples of untargeted generative adversarial examples (w/o noise) against certified defenses on MNIST. Green and red borders indicate success/failure respectively, according to MTurk results. The annotation in upper-left corner of each image represents the classifier's prediction.}
\end{figure}
\vfill
\newpage

\begin{figure}
	\centering
	\subfigure[success rates on MNIST]{\includegraphics[width=0.4\textwidth]{mnist_madry_adv_targeted_matrix_noisy.png}}%
	\subfigure[success rates on SVHN]{\includegraphics[width=0.4\textwidth]{svhn_resnet_adv_targeted_matrix_noisy.png}}
	\caption{The success rates (\%) of our targeted generative adversarial attack with noise-augmentation.}
\end{figure}

\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{mnist_madry_adv_targeted_large_plot.jpg}
	\caption{(Extended plot of \figref{fig:mnist_sample}) Random samples of targeted generative adversarial examples (w/o noise) on MNIST. Green border indicates that the image is voted legitimate by MTurk workers, and red border means the label given by workers (as shown in the upper left corner) disagrees with the image's source class.}
\end{figure}

\newpage
\vspace*{\fill}
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{mnist_madry_adv_targeted_noisy_large_plot.jpg}
	\caption{Random samples of targeted generative adversarial examples (w/ noise) on MNIST. Green border indicates that the image is voted legitimate by MTurk workers, and red border means the label given by workers (as shown in the upper left corner) disagrees with the image's source class.}
\end{figure}
\vfill

\newpage
\vspace*{\fill}
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{svhn_resnet_adv_targeted_large_plot.png}
	\caption{(Extended plot of \figref{fig:svhn_sample}) Random samples of targeted generative adversarial examples (w/o noise) on SVHN. Green border indicates that the image is voted legitimate by MTurk workers, and red border means the label given by workers (as shown in the upper left corner) disagrees with the image's source class.}
\end{figure}
\vfill

\newpage
\vspace*{\fill}
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{svhn_resnet_adv_targeted_noisy_large_plot.png}
	\caption{Random samples of targeted generative adversarial examples (w/ noise) on SVHN. Green border indicates that the image is voted legitimate by MTurk workers, and red border means the label given by workers (as shown in the upper left corner) disagrees with the image's source class.}
\end{figure}
\vfill

\clearpage
\vspace*{\fill}
\begin{figure}
	\centering
	\includegraphics[width=\textwidth]{celebA_resnet_adv_targeted_large_plot.jpg}
	\caption{(Extended plot of \figref{fig:2}) Sampled generative adversarial examples (w/o noise) for fooling the classifier to misclassify a female as male (left) and the other way around (right). Green, red borders and annotations have the same meanings as in \figref{fig:1}, except ``F'' is short for ``Female'' and ``M'' is short for ``Male''.}
\end{figure}
\vfill

\newpage
\vspace*{\fill}
\begin{figure}[H]
	\centering
	\includegraphics[width=\textwidth]{celebA_resnet_adv_targeted_noisy_large_plot.jpg}
	\caption{Sampled generative adversarial examples (w/ noise) for fooling the classifier to misclassify a female as male (left) and the other way around (right). Green, red borders and annotations have the same meanings as in \figref{fig:1}, except ``F'' is short for ``Female'' and ``M'' is short for ``Male''.}
\end{figure}

\section{MTurk web interfaces}\label{app:amt}
The MTurk web interfaces used for labeling our generative adversarial examples are depicted in \figref{fig:mturk}. The A/B test interface used in Section~\ref{sec:detection} is shown in \figref{fig:mturkab}. In addition, \figref{fig:barplot} visualizes the uncertainty of MTurk annotators for labeling generative adversarial examples, which indicates that more than 40\%-50\% generative adversarial examples (depending on the dataset) get all of their 5 annotators agreed on one label. 

\begin{figure}
	\centering
	\subfigure[The MTurk web interface for MNIST and SVHN.]{\includegraphics[width=0.8\textwidth]{mturk1.png}}
	
	\subfigure[The MTurk web interface for CelebA.]{\includegraphics[width=0.8\textwidth]{mturk2.png}}
	\caption{MTurk web interfaces for labeling generative adversarial examples.}\label{fig:mturk}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.8\textwidth]{mturk3.png}
	\caption{MTurk web interfaces for A/B test on MNIST.}\label{fig:mturkab}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{uncertainties.png}
	\caption{The distribution of number of agreed votes for each image. For example, the red bar on top of 5 means around 55\% generative adversarial examples on CelebA dataset are voted the same label by all 5 MTurk annotators.}\label{fig:barplot}
\end{figure}



